Deep Investigation of Cross-Language Plagiarism Detection Methods

This paper is a deep investigation of cross-language plagiarism detection methods on a new recently introduced open dataset, which contains parallel and comparable collections of documents with multiple characteristics (different genres, languages and sizes of texts). We investigate cross-language plagiarism detection methods for 6 language pairs on 2 granularities of text units in order to draw robust conclusions on the best methods while deeply analyzing correlations across document styles and languages.

==> BUCC - pour arXiv/forest/README <==
LaTeX package: forest [2015/07/15 v1.0.10 Drawing (linguistic) trees]

Copyright (c) 2015 Saso Zivanovic
                   (Sa\v{s}o \v{Z}ivanovi\'{c})
saso.zivanovic@guest.arnes.si


ABSTRACT

`forest' is a pgf/tikz-based package for drawing linguistic (and other
kinds of) trees. Its main features are:
- a packing algorithm which can produce very compact trees;
- a user-friendly interface consisting of the familiar bracket
encoding of trees plus the key--value interface to option-setting;
- many tree-formatting options, with control over option values of
individual nodes and mechanisms for their manipulation;
- the possibility to decorate the tree using the full power of pgf/tikz;
- an externalization mechanism sensitive to code-changes.


LICENSE

This work may be distributed and/or modified under the
conditions of the LaTeX Project Public License, either version 1.3
of this license or (at your option) any later version.
The latest version of this license is in

http://www.latex-project.org/lppl.txt

and version 1.3 or later is part of all distributions of LaTeX
version 2005/12/01 or later.



==> forest/README <==
LaTeX package: forest [2015/07/15 v1.0.10 Drawing (linguistic) trees]

Copyright (c) 2015 Saso Zivanovic
                   (Sa\v{s}o \v{Z}ivanovi\'{c})
saso.zivanovic@guest.arnes.si


ABSTRACT

`forest' is a pgf/tikz-based package for drawing linguistic (and other
kinds of) trees. Its main features are:
- a packing algorithm which can produce very compact trees;
- a user-friendly interface consisting of the familiar bracket
encoding of trees plus the key--value interface to option-setting;
- many tree-formatting options, with control over option values of
individual nodes and mechanisms for their manipulation;
- the possibility to decorate the tree using the full power of pgf/tikz;
- an externalization mechanism sensitive to code-changes.


LICENSE

This work may be distributed and/or modified under the
conditions of the LaTeX Project Public License, either version 1.3
of this license or (at your option) any later version.
The latest version of this license is in

http://www.latex-project.org/lppl.txt

and version 1.3 or later is part of all distributions of LaTeX
version 2005/12/01 or later.


